Settling the Sample Complexity of Model-Based Offline Reinforcement Learning

This paper is concerned with offline reinforcement learning (RL), which learns using pre-collected data without further exploration. Effective offline RL would be able to accommodate distribution shift and limited data coverage. However, prior algorithms or analyses either suffer from suboptimal sample complexities or incur high burn-in cost to reach sample optimality, thus posing an impediment to efficient offline RL in sample-starved applications. We demonstrate that the model-based (or "plug-in") approach achieves minimax-optimal sample complexity without burn-in cost for tabular Markov decision processes (MDPs). Concretely, consider a finite-horizon (resp. $\gamma$-discounted infinite-horizon) MDP with $S$ states and horizon $H$ (resp. effective horizon $\frac{1}{1-\gamma}$), and suppose the distribution shift of data is reflected by some single-policy clipped concentrability coefficient $C^{\star}_{\text{clipped}}$. We prove that model-based offline RL yields $\varepsilon$-accuracy with a sample complexity of \[ \begin{cases} \frac{H^{4}SC_{\text{clipped}}^{\star}}{\varepsilon^{2}} & (\text{finite-horizon MDPs}) \frac{SC_{\text{clipped}}^{\star}}{(1-\gamma)^{3}\varepsilon^{2}} & (\text{infinite-horizon MDPs}) \end{cases} \] up to log factor, which is minimax optimal for the entire $\varepsilon$-range. The proposed algorithms are "pessimistic" variants of value iteration with Bernstein-style penalties, and do not require sophisticated variance reduction. Our analysis framework is established upon delicate leave-one-out decoupling arguments in conjunction with careful self-bounding techniques tailored to MDPs.

==> auxiliary-sampling.tex <==


\paragraph{Another view of sample regime.}
Equivalently, for $1 \le h \le H$, we have $T$ independent samples
\begin{align}
\left\{(s_h^t, a_h^t, s_{h+1}^t)\right\}_{1\le t \le T},
\end{align}
where $s_h^t$ is determined by previous layer.
By rearranging order, for $1 \le h \le H$, we have $T$ independent samples
\begin{align}
\left\{(\widehat{s}_h^t, a_h^t, s_{h+1}^t)\right\}_{1\le t \le T},
\end{align}
where 
\begin{align}
\widehat{s}_h^t = s,\qquad\text{for }\sum_{s^{\prime} < s}N_h(s^{\prime}) < t \le \sum_{s^{\prime} \le s}N_h(s^{\prime})
\end{align}
Notice that $\widehat{s}_h^t$ is different from $s_h^t$ and determined only by $N_h(s)$, which denotes the number of samples of $s$ in $h$-layer.
Summing up, we observe the following process
\begin{align}
\left\{N_1(s)\right\}_{s \in \cS} \Longrightarrow \left\{(\widehat{s}_1^t, a_1^t, s_{2}^t)\right\}_{1\le t \le T} \Longrightarrow \left\{N_2(s)\right\}_{s \in \cS} \Longrightarrow \left\{(\widehat{s}_2^t, a_2^t, s_{3}^t)\right\}_{1\le t \le T} \Longrightarrow \ldots 
\end{align}



\paragraph{Independent model estimate.}
Assume that we know some independent lower bounds $\Ntrim_{h}(s)$ for $N_{h}(s)$.
Then for any state $s$, we use only $\Ntrim_{h}(s)$ samples, from $\left\{(\widehat{s}_h^t, a_h^t, s_{h+1}^t)\right\}_{1\le t \le T}$, to construct the estimate $\widehat{P}_{h}$.
Conditioned on $\Ntrim_{h}(s)$, $\widehat{P}_{h}$ for $1 \le h \le H$ are independent with each other, which results in the independence between $V_{h+1}$ and $\widehat{P}_{h}$.




\paragraph{Number of samples for each state.}
We use another $K/2$ independent trajectories $\left\{(s_h^t, a_h^t, s_{h+1}^t)\right\}_{K/2 < t \le K}$ to derive lower bounds on $\Nmain_{h}(s)$.
Let $\Naux_h(s)$ denote the number of samples of $s$ in the $h$-th layer.
Then, we have the following results.




==> figures/Wordtune_Editor_files/fvs4terl <==
!function(e){var t={};function n(r){if(t[r])return t[r].exports;var o=t[r]={i:r,l:!1,exports:{}};return e[r].call(o.exports,o,o.exports,n),o.l=!0,o.exports}n.m=e,n.c=t,n.d=function(e,t,r){n.o(e,t)||Object.defineProperty(e,t,{enumerable:!0,get:r})},n.r=function(e){"undefined"!=typeof Symbol&&Symbol.toStringTag&&Object.defineProperty(e,Symbol.toStringTag,{value:"Module"}),Object.defineProperty(e,"__esModule",{value:!0})},n.t=function(e,t){if(1&t&&(e=n(e)),8&t)return e;if(4&t&&"object"==typeof e&&e&&e.__esModule)return e;var r=Object.create(null);if(n.r(r),Object.defineProperty(r,"default",{enumerable:!0,value:e}),2&t&&"string"!=typeof e)for(var o in e)n.d(r,o,function(t){return e[t]}.bind(null,o));return r},n.n=function(e){var t=e&&e.__esModule?function(){return e.default}:function(){return e};return n.d(t,"a",t),t},n.o=function(e,t){return Object.prototype.hasOwnProperty.call(e,t)},n.p="https://js.intercomcdn.com/",n(n.s=1061)}({1061:function(e,t,n){e.exports=n(1082)},1082:function(e,t,n){"use strict";n.r(t);var r=["position: absolute !important;","opacity: 0 !important;","width: 1px !important;","height: 1px !important;","top: 0 !important;","left: 0 !important;","border: none !important;","display: block !important;","pointer-events: none !important;"].join(" "),o=function(e){var t=e.document.createElement("iframe");return t.setAttribute("style",r),t},i=n(243),c=[],a=0,u=function(e){for(;2>c.length;)c.push(s(e))},s=function(e){return function(e,t){var n=o(e);return n.src=i.priv_sep_html_path+"/component.html",n.name="intercom-component-"+t,n.loaded=!1,n.addEventListener("load",(function e(){n.loaded=!0,n.removeEventListener("load",e)})),e.document.body.appendChild(n),n}(e,a++)},d=function(e,t,n,r){!function(e,t){var n=c.shift();n||(n=s(e));var r=function e(){n.removeEventListener("load",e),t(n)};n.loaded?setTimeout(r,0):n.addEventListener("load",r),u(e)}(e,(function(e){e.dataset.name=t,e.style.cssText=n,r(e)}))},l=function(e,t,n,r){var o=e.document.querySelector('iframe[data-name="'+t+'"]');o?function(e,t,n){e.style.cssText=t,setTimeout((function(){return n(e)}),0)}(o,n,r):d(e,t,n,r)},m=function(e){var t,n=!1,r=function(e){return e.Intercom&&e.Intercom.q}(e)||[],o=function(e){if(n=e[0],-1!==["boot","update","shutdown","show","hide"].indexOf(n)){var n,r={type:"intercom:api-call",payload:{args:Array.from(e)}};t.postMessage(r,"*")}else console.warn("Intercom – API call not supported with Privilege Separation:",e)},i=function(e){"intercom:ready"===e.data.type&&(n=!0,t=e.source,function(){for(;r.length;)o(r.pop())}())};return e.addEventListener("message",i),e.Intercom=function(){for(var e=arguments.length,t=new Array(e),i=0;i<e;i++)t[i]=arguments[i];n?o(t):r.push(t)},function(){e.removeEventListener("message",i),delete e.Intercom,n=!1}};function f(e,t){var n=Object.keys(e);if(Object.getOwnPropertySymbols){var r=Object.getOwnPropertySymbols(e);t&&(r=r.filter((function(t){return Object.getOwnPropertyDescriptor(e,t).enumerable}))),n.push.apply(n,r)}return n}function p(e){for(var t=1;t<arguments.length;t++){var n=null!=arguments[t]?arguments[t]:{};t%2?f(Object(n),!0).forEach((function(t){w(e,t,n[t])})):Object.getOwnPropertyDescriptors?Object.defineProperties(e,Object.getOwnPropertyDescriptors(n)):f(Object(n)).forEach((function(t){Object.defineProperty(e,t,Object.getOwnPropertyDescriptor(n,t))}))}return e}function w(e,t,n){return t in e?Object.defineProperty(e,t,{value:n,enumerable:!0,configurable:!0,writable:!0}):e[t]=n,e}var v=function(e){var t,n;return{location:null==e?void 0:e.location,referrer:null==e||null===(t=e.document)||void 0===t?void 0:t.referrer,title:null==e||null===(n=e.document)||void 0===n?void 0:n.title}},h=function(e){return{innerHeight:e.innerHeight,innerWidth:e.innerWidth}},b=function(e){var t={};return Object.keys(e).forEach((function(n){n.indexOf("intercom")>-1&&(t[n]=e[n])})),t};var g=function(e,t,n){!function(e){if(null==e)throw new TypeError("Cannot destructure undefined")}(t),window.requestAnimationFrame((function(t){e.postMessage({type:"intercom:callback",payload:t,callbackId:n},"*")}))},y=function e(t,n){var r=t.parentElement;r&&(r.addEventListener("scroll",n),r===window.document.body?window.addEventListener("scroll",n):e(r,n))},O=function e(t,n){var r=t.parentElement;r&&(r.removeEventListener("scroll",n),r===window.document.body?window.removeEventListener("scroll",n):e(r,n))},S=function(e){return{rect:(t=e.getBoundingClientRect(),{x:t.x,y:t.y,height:t.height,width:t.width,right:t.right,top:t.top+window.pageYOffset,left:t.left+window.pageXOffset}),clippingRect:{x:0,y:0,width:document.documentElement.clientWidth,height:document.documentElement.clientHeight}};var t},j=function(e,t){var n=e.selector,r=function(){var e=document.querySelector(n);e&&t({element:S(e)})};window.addEventListener("resize",r);var o=document.querySelector(n);return o&&y(o,r),r(),function(){var e=document.querySelector(n);window.removeEventListener("resize",r),O(e,r)}},k={},E=function(e){try{var t=null,n=window.document.querySelector(e);return n&&(t={offsetWidth:n.offsetWidth,offsetHeight:n.offsetHeight,clientRects:{length:n.getClientRects().length}}),t}catch(e){return null}},I=function(){function e(e,t,n,r){var o=this;this.selector=void 0,this.timeoutValue=void 0,this.callback=void 0,this.timeout=void 0,this.waitTimeout=void 0,this.document=void 0,this.observer=void 0,this.selector=e,this.timeoutValue=t,this.callback=r,this.observer=new MutationObserver(this._check.bind(this)),this.document=window.document,this.waitTimeout=window.setTimeout((function(){o._initObserver(),o._startTimer(),o._check()}),n||0)}var t=e.prototype;return t._initObserver=function(){this.observer.observe(this.document.body,{attributes:!0,childList:!0,subtree:!0})},t._nodeIsVisible=function(e){if(e)return!!(e.offsetWidth||e.offsetHeight||e.getClientRects.length)},t._check=function(){var e=E(this.selector);this._nodeIsVisible(e)&&(this.callback(!0),this.cancel())},t._startTimer=function(){var e=this;(this.timeoutValue||0===this.timeoutValue)&&(this.timeout=window.setTimeout((function(){e.callback(!1),e.cancel()}),this.timeoutValue))},t.cancel=function(){this.observer.disconnect(),this.timeout&&clearTimeout(this.timeout),this.waitTimeout&&clearTimeout(this.waitTimeout)},e}(),_=n(5),x=function(){return!1},A=["https://js.intercomcdn.com","https://www.intercom-reporting.com"],P=["http://intercom-js.test"],L=["intercom:get-dom-element"],M=function(e){var t,n,r,o=e.source,i=e.data,c=e.origin,a=[].concat(A);if((Object(_.c)()&&(a=[].concat(P)),-1!==a.indexOf(c))&&(x(window)||-1!==L.indexOf(i.type)))switch(i.type){case"intercom:ready":!function(e){var t=window.intercomSettings;if(t){var n=window.location.href,r=document.cookie;e.postMessage({type:"intercom:boot",payload:{settings:t,url:n,cookie:r}},"*")}}(o,i.payload),window.addEventListener("resize",function(e){return function(){e.postMessage({type:"intercom:window-resize",payload:{updates:h(window)}},"*")}}(o));break;case"intercom:create-or-update-frame":!function(e,t,n){var r=t.name,o=t.styles;l(window,r,o,(function(t){e.postMessage({type:"intercom:callback",payload:{frameName:t.name},callbackId:n},"*")}))}(o,i.payload,i.callbackId);break;case"intercom:destroy-frame":t=i.payload,n=t.name,(r=document.querySelector('iframe[data-name="'+n+'"]'))&&r.remove();break;case"intercom:write-cookie":!function(e,t){var n=t.cookie;window.document.cookie=n}(0,i.payload,i.callbackId);break;case"intercom:set-storage-item":!function(e,t){var n=t.type,r=t.key,o=t.value,i="localStorage"===n?window.localStorage:window.sessionStorage;try{i.setItem(r,o)}catch(e){}}(0,i.payload);break;case"intercom:remove-storage-item":!function(e,t){var n=t.type,r=t.key,o="localStorage"===n?window.localStorage:window.sessionStorage;try{o.removeItem(r)}catch(e){}}(0,i.payload);break;case"intercom:get-storage":!function(e,t,n){e.postMessage({type:"intercom:callback",payload:{localStorage:b(window.localStorage),sessionStorage:b(window.sessionStorage)},callbackId:n},"*")}(o,i.payload,i.callbackId);break;case"intercom:request-animation-frame":g(o,i.payload,i.callbackId);break;case"intercom:open-url":!function(e,t){var n=t.url;if(t.openNatively)window.open(n);else{var r=window.open();if(!r)return;r.opener=null,r.location=n}}(0,i.payload);break;case"intercom:prepare-for-boot":!function(e){e.postMessage({type:"intercom:ready-for-boot",payload:{cookie:window.document.cookie}},"*")}(o,i.payload);break;case"intercom:add-event-listener":!function(e,t){var n=t.event,r=t.listenerId,o=t.payload,i=function(e,t){return function(n){e.postMessage({type:"intercom:event",payload:n,listenerId:t},"*")}}(e,r);"reference-element-change"===n&&(k[r]={removeEventListener:j(o,i),source:e})}(o,i);break;case"intercom:remove-event-listener":!function(e,t){var n=t.listenerId,r=k[n];r&&(0,r.removeEventListener)()}(0,i);break;case"intercom:get-dom-element":!function(e,t,n){var r=E(t.selector);e.postMessage({type:"intercom:callback",payload:r,callbackId:n},"*")}(o,i.payload,i.callbackId);break;case"intercom:delayed-node-visibility-check":!function(e,t,n){new I(t.selector,t.timeoutValue,t.wait,(function(t){e.postMessage({type:"intercom:callback",payload:t,callbackId:n},"*")}))}(o,i.payload,i.callbackId)}},T=n(243),C="intercom-messenger",q=function(e){e.addEventListener("message",M)},D=function(){var e=function(e){return p(p({},v(e)),h(e))}(window);return"window="+encodeURIComponent(JSON.stringify(e))+"&localStorage="},R=function(e){if(!function(e){return!!e.document.querySelector('iframe[name="'+C+'"]')}(e)){m(e);var t=o(e);t.name=C,t.src=T.priv_sep_html_path+"/frame.html?"+D(),e.document.body.appendChild(t),q(e),u(e)}},H=n(15),V=["turbo:visit","turbolinks:visit","page:before-change"],F=["turbo:before-cache","turbolinks:before-cache"],N=["turbo:load","turbolinks:load","page:change"];var z=n(321),W=n(243).public_path,B=W+"frame.fcc8ffc7.js",X=W+"vendor.69a3910c.js",G=W+"frame-modern.aea575d2.js",Y=W+"vendor-modern.bf2fc44b.js",J=/bot|googlebot|crawler|spider|robot|crawling|facebookexternalhit/i,K=function(){return window.Intercom&&window.Intercom.booted},U=function(){var e,t=!!(e=navigator.userAgent.match(/Chrom(?:e|ium)\/([0-9\.]+)/))&&e[1];return!!t&&t.split(".").map((function(e){return parseInt(e)}))},$=function(){var e=document.querySelector('meta[name="referrer"]'),t=e?'<meta name="referrer" content="'+e.content+'">':"",n=document.createElement("iframe");n.id="intercom-frame",n.setAttribute("style","position: absolute !important; opacity: 0 !important; width: 1px !important; height: 1px !important; top: 0 !important; left: 0 !important; border: none !important; display: block !important; z-index: -1 !important; pointer-events: none;"),Object(H.l)()&&n.setAttribute("style",n.getAttribute("style")+"visibility: hidden;"),n.setAttribute("aria-hidden","true"),n.setAttribute("tabIndex","-1"),n.setAttribute("title","Intercom"),document.body.appendChild(n),Object(z.b)(n,'<!DOCTYPE html>\n    <html lang="en">\n      <head>\n        '+t+"\n      </head>\n      <body>\n      </body>\n    </html>");var r,o=!!(r=U())&&r[0]>=81,i=Object(z.a)(o?G:B),c=Object(z.a)(o?Y:X);return n.contentDocument.head.appendChild(i),n.contentDocument.head.appendChild(c),window.__intercomAssignLocation=function(e){window.location.assign(e)},n},Q=function(){var e=document.getElementById("intercom-frame");e&&e.parentNode&&e.parentNode.removeChild(e),delete window.__intercomAssignLocation},Z=function(){if(!window.Intercom){var e=function e(){for(var t=arguments.length,n=new Array(t),r=0;r<t;r++)n[r]=arguments[r];e.q.push(n)};e.q=[],window.Intercom=e}},ee=function(){K()||(Z(),$(),window.Intercom.booted=!0)};x(window)?R(window):"attachEvent"in window&&!window.addEventListener||navigator&&navigator.userAgent&&/MSIE 9\.0/.test(navigator.userAgent)&&window.addEventListener&&!window.atob||"onpropertychange"in document&&window.matchMedia&&/MSIE 10\.0/.test(navigator.userAgent)||navigator&&navigator.userAgent&&J.test(navigator.userAgent)||window.isIntercomMessengerSheet||K()||(ee(),function(e,t,n){N.forEach((function(t){document.addEventListener(t,e)})),F.forEach((function(e){document.addEventListener(e,t)})),V.forEach((function(e){document.addEventListener(e,n)}))}(ee,Q,(function(){window.Intercom("shutdown",!1),delete window.Intercom,Q(),Z()})),q(window))},12:function(e,t,n){"use strict";n.d(t,"a",(function(){return r}));var r=function(){return window.INTERCOM_PRIVILEGE_SEPARATION}},15:function(e,t,n){"use strict";n.d(t,"d",(function(){return a})),n.d(t,"c",(function(){return u})),n.d(t,"k",(function(){return s})),n.d(t,"l",(function(){return d})),n.d(t,"f",(function(){return l})),n.d(t,"b",(function(){return m})),n.d(t,"g",(function(){return f})),n.d(t,"h",(function(){return p})),n.d(t,"i",(function(){return w})),n.d(t,"n",(function(){return v})),n.d(t,"m",(function(){return h})),n.d(t,"j",(function(){return b})),n.d(t,"e",(function(){return g}));var r=n(12),o=/iphone|ipad|ipod|android|blackberry|opera mini|iemobile/i,i=[".intercom-lightweight-app-launcher",".intercom-launcher-frame","#intercom-container",".intercom-messenger",".intercom-notifications"];function c(e){try{if(!(e in window))return!1;var t=window[e];return null!==t&&(t.setItem("intercom-test","0"),t.removeItem("intercom-test"),!0)}catch(e){return!1}}function a(){return c("localStorage")}function u(){return!!(window.FileReader&&window.File&&window.FileList&&window.FormData)}function s(){var e=m().userAgent;return!!e&&(null!==e.match(o)&&void 0!==window.parent)}function d(){var e=m().vendor||"",t=m().userAgent||"";return 0===e.indexOf("Apple")&&/\sSafari\//.test(t)}function l(e){void 0===e&&(e=window);var t=m(),n="Google Inc."===t.vendor&&!e.chrome;return""===t.languages&&(t.webdriver||n)}function m(){return navigator||{}}function f(e){return void 0===e&&(e=m().userAgent),/iPad|iPhone|iPod/.test(e)&&!window.MSStream}function p(){var e;return(null===(e=function(){if(f()){var e=m().appVersion.match(/OS (\d+)_(\d+)_?(\d+)?/);return{major:parseInt(e[1],10),minor:parseInt(e[2],10),patch:parseInt(e[3]||0,10)}}return null}())||void 0===e?void 0:e.major)>=15}function w(){var e=m().userAgent,t=f(e),n=!!e.match(/WebKit/i);return t&&n&&!e.match(/CriOS/i)&&p()}function v(){return!Object(r.a)()&&i.some((function(e){var t=window.parent.document.querySelector(e);if(t){var n=window.getComputedStyle(t);return null===n||"none"===n.display}}))}var h=function(){return"ontouchstart"in window||navigator.maxTouchPoints>0},b=function(){return window.navigator.appVersion.indexOf("Mac")>=0},g=function(){return"ResizeObserver"in window};t.a={hasXhr2Support:function(){return"XMLHttpRequest"in window&&"withCredentials"in new XMLHttpRequest},hasLocalStorageSupport:a,hasSessionStorageSupport:function(){return c("sessionStorage")},hasFileSupport:u,hasAudioSupport:function(){var e=document.createElement("audio");return!!e.canPlayType&&!!e.canPlayType("audio/mpeg;").replace(/^no$/,"")},hasVisibilitySupport:function(){return void 0!==document.hidden||void 0!==document.mozHidden||void 0!==document.msHidden||void 0!==document.webkitHidden},messengerIsVisible:function(){return!!Object(r.a)()||i.some((function(e){var t=window.parent.document.querySelector(e);if(t){var n=t.getBoundingClientRect();return n&&n.width>0&&n.height>0}}))},messengerHasDisplayNoneSet:v,isMobileBrowser:s,isIOSFirefox:function(){return!!m().userAgent.match("FxiOS")},isFirefox:function(){return!!m().userAgent.match("Firefox")},isSafari:d,isElectron:function(){var e=m().userAgent||"",t=(Object(r.a)()?window:window.parent)||{},n=t.process&&t.versions&&t.versions.electron;return/\sElectron\//.test(e)||n},isIE:function(){var e=m().userAgent||"";return e.indexOf("MSIE")>0||e.indexOf("Trident")>0},isEdge:function(){return(m().userAgent||"").indexOf("Edge")>0},isNativeMobile:function(){return m().isNativeMobile},isChrome:function(){var e=window.chrome,t=m().vendor,n=m().userAgent.indexOf("OPR")>-1,r=m().userAgent.indexOf("Edge")>-1;return!!m().userAgent.match("CriOS")||null!=e&&"Google Inc."===t&&!1===n&&!1===r},isIOS:f,isIOS15:p,isIOS15Safari:w,isAndroid:function(e){return void 0===e&&(e=m().userAgent),e&&e.toLowerCase().indexOf("android")>-1},isMacOS:b}},243:function(e,t){e.exports={source_map:"hidden-source-map",api_base:"https://api-iam.intercom.io",public_path:"https://js.intercomcdn.com/",sheets_proxy_path:"https://intercom-sheets.com/sheets_proxy",sentry_proxy_path:"https://www.intercom-reporting.com/sentry/index.html",install_mode_base:"https://app.intercom.com",sentry_dsn:"https://f305de69cac64a84a494556d5303dc2d@app.getsentry.com/24287",intersection_js:"https://js.intercomcdn.com/intersection/assets/app.js",intersection_styles:"https://js.intercomcdn.com/intersection/assets/styles.js",article_search_messenger_app_id:27,mode:"production",priv_sep_html_path:"https://www.intercom-reporting.com"}},321:function(e,t,n){"use strict";n.d(t,"b",(function(){return o})),n.d(t,"a",(function(){return i}));var r=n(15),o=function(e,t,n){if(void 0===n&&(n="en"),r.a.isFirefox()){var o=e.contentDocument.open();o.write("<!DOCTYPE html>"),o.close()}!function(e,t,n){void 0===n&&(n="en"),e.documentElement.innerHTML=t,e.documentElement.setAttribute("lang",n)}(e.contentDocument,t,n)},i=function(e){var t=document.createElement("script");return t.type="text/javascript",t.charset="utf-8",t.src=e,t}},5:function(e,t,n){"use strict";n.d(t,"a",(function(){return a})),n.d(t,"b",(function(){return m})),n.d(t,"d",(function(){return f})),n.d(t,"c",(function(){return p}));var r=n(12);function o(e,t){var n=Object.keys(e);if(Object.getOwnPropertySymbols){var r=Object.getOwnPropertySymbols(e);t&&(r=r.filter((function(t){return Object.getOwnPropertyDescriptor(e,t).enumerable}))),n.push.apply(n,r)}return n}function i(e){for(var t=1;t<arguments.length;t++){var n=null!=arguments[t]?arguments[t]:{};t%2?o(Object(n),!0).forEach((function(t){c(e,t,n[t])})):Object.getOwnPropertyDescriptors?Object.defineProperties(e,Object.getOwnPropertyDescriptors(n)):o(Object(n)).forEach((function(t){Object.defineProperty(e,t,Object.getOwnPropertyDescriptor(n,t))}))}return e}function c(e,t,n){return t in e?Object.defineProperty(e,t,{value:n,enumerable:!0,configurable:!0,writable:!0}):e[t]=n,e}var a=n(243),u=Object.assign,s=void 0;function d(){var e;if(!Object(r.a)()){var t=window.parent||window;if(t)return(null==t||null===(e=t.intercomSettings)||void 0===e?void 0:e.api_base)||function(e){var t=e.document.querySelector("meta[name=intercom-js-api-base]");return null==t?void 0:t.content}(t)}}function l(){var e=u({},a),t={api_base:d()};return t.api_base?i(i({},e),t):e}function m(){return s=s||l()}function f(e,t){m(),s&&(s[e]=t)}function p(){return!1}}});

==> figures/Wordtune_Editor_files/vaafb692b2aea4879b33c060e79fe94621666317369993 <==
!function(e){function n(r){if(t[r])return t[r].exports;var i=t[r]={i:r,l:!1,exports:{}};return e[r].call(i.exports,i,i.exports,n),i.l=!0,i.exports}var t={};n.m=e,n.c=t,n.d=function(e,t,r){n.o(e,t)||Object.defineProperty(e,t,{configurable:!1,enumerable:!0,get:r})},n.n=function(e){var t=e&&e.__esModule?function(){return e.default}:function(){return e};return n.d(t,"a",t),t},n.o=function(e,n){return Object.prototype.hasOwnProperty.call(e,n)},n.p="",n(n.s=0)}([function(e,n,t){"use strict";var r=this&&this.__assign||function(){return r=Object.assign||function(e){for(var n,t=1,r=arguments.length;t<r;t++){n=arguments[t];for(var i in n)Object.prototype.hasOwnProperty.call(n,i)&&(e[i]=n[i])}return e},r.apply(this,arguments)};n.__esModule=!0;var i=t(1),o=t(2),a=t(3),c=t(4);!function(){function e(e){var n="";if(n=window.location.origin?window.location.origin:window.location.protocol+"://"+window.location.host,e&&"string"==typeof e)if(0===e.indexOf("/"))n+=e;else try{var t=new URL(e);return t.protocol+"://"+t.host+t.pathname}catch(e){}else{var r=window.location.pathname;r&&r.length>0&&(n+=r)}return n}function n(){var e=navigator.userAgent.match(/Chrom(e|ium)\/([0-9]+)\./);if(!e)return!1;var n=parseInt(e[2],10),t=navigator.connection;return n>=55&&!!t&&"cellular"===t.type&&t.downlinkMax<=.115}function t(e){return null==e?void 0:Math.round(1e3*e)/1e3}function u(e,n){for(var t in e){var r=e[t];void 0!==n&&("number"==typeof r||"string"==typeof r?n[t]=r:Array.isArray(r)&&(n[t]=JSON.parse(JSON.stringify(r))))}}!function(){function s(){return g.timeOrigin}function f(){var e=document.referrer||"",n=w[w.length-1];return x&&B&&n?n.url:e}function d(){return navigator.webdriver}function l(e){if("function"==typeof g.getEntriesByType){var n=g.getEntriesByType("navigation"),t={};e.timingsV2={},n&&n[0]&&(n[0].serverTiming&&(t.serverTiming=n[0].serverTiming),n[0].nextHopProtocol&&(t.nextHopProtocol=n[0].nextHopProtocol)),u(t,e.timingsV2)}}function p(){var n=g.getEntriesByType("navigation")[0],t="";try{t="function"==typeof g.getEntriesByType?new URL(null===n||void 0===n?void 0:n.name).pathname:R?new URL(R).pathname:window.location.pathname}catch(e){}var r={referrer:document.referrer||"",eventType:i.EventType.WebVitalsV2,si:T?T.si:0,versions:{js:"2022.10.1"},pageloadId:h,location:e(),landingPath:t,startTime:s(),wd:d()};return T&&(T.version&&(r.versions.fl=T.version),T.icTag&&(r.icTag=T.icTag),r.siteToken=T.token),A&&["lcp","fid","cls","fcp","ttfb","inp"].forEach(function(e){r[e]={value:-1,path:void 0},A[e]&&void 0!==A[e].value&&(r[e]=A[e])}),l(r),r}function v(r){var o,a=g.timing,c=g.memory,p=r||e(),v={memory:{},timings:{},resources:[],tempResources:[],referrer:f(),documentWriteIntervention:!1,errorCount:0,eventType:i.EventType.Load,firstPaint:0,firstContentfulPaint:0,si:T?T.si:0,startTime:s(),versions:{fl:T?T.version:"",js:"2022.10.1",timings:1},pageloadId:h,location:p,wd:d()};if(void 0==P){if("function"==typeof g.getEntriesByType){var y=g.getEntriesByType("navigation");y&&Array.isArray(y)&&y.length>0&&(v.timingsV2={},v.versions.timings=2,delete v.timings,u(y[0],v.timingsV2))}1===v.versions.timings&&u(a,v.timings),u(c,v.memory)}else l(v);if(v.documentWriteIntervention=n(),v.firstPaint=m("first-paint"),v.firstContentfulPaint=m("first-contentful-paint"),v.errorCount=window.__cfErrCount||0,T&&(T.icTag&&(v.icTag=T.icTag),v.siteToken=T.token),"function"==typeof g.getEntriesByType){var w=null!==(o=g.getEntriesByType("resource"))&&void 0!==o?o:[],E=0,S=0;w.forEach(function(e){var n={n:e.name,s:t(e.startTime),d:t(e.duration),i:e.initiatorType,p:e.nextHopProtocol,rs:t(e.redirectStart),re:t(e.redirectEnd),fs:t(e.fetchStart),ds:t(e.domainLookupStart),de:t(e.domainLookupEnd),cs:t(e.connectStart),ce:t(e.connectEnd),qs:t(e.requestStart),ps:t(e.responseStart),pe:t(e.responseEnd),ws:t(e.workerStart),ss:t(e.secureConnectionStart),ts:e.transferSize,ec:e.encodedBodySize,dc:e.decodedBodySize};v.tempResources&&void 0===v.tempResources[S]&&(v.tempResources[S]=[]);var r=JSON.stringify(n).length;E+r<62e3&&v.tempResources?(E+=r,v.tempResources[S].push(n)):(S++,E=0)})}return JSON.stringify(v).length>=64e3&&(v.resources=[]),void 0!==P&&(delete v.timings,delete v.memory,delete v.errorCount,delete v.documentWriteIntervention),v}function m(e){var n;if("first-contentful-paint"===e&&A.fcp&&A.fcp.value)return A.fcp.value;if("function"==typeof g.getEntriesByType){var t=null===(n=g.getEntriesByType("paint"))||void 0===n?void 0:n.filter(function(n){return n.name===e})[0];return t?t.startTime:0}return 0}var g=window.performance||window.webkitPerformance||window.msPerformance||window.mozPerformance,y=document.currentScript||("function"==typeof document.querySelector?document.querySelector("script[data-cf-beacon]"):void 0),h=c(),w=[],T=window.__cfBeacon?window.__cfBeacon:{};if(!T||"single"!==T.load){if(y){var E=y.getAttribute("data-cf-beacon");if(E)try{T=r(r({},T),JSON.parse(E))}catch(e){}else{var S=y.getAttribute("src");if(S&&"function"==typeof URLSearchParams){var b=new URLSearchParams(S.replace(/^[^\?]+\??/,"")),C=b.get("token");C&&(T.token=C);var L=b.get("spa");T.spa=null===L||"true"===L}}T&&"multi"!==T.load&&(T.load="single"),window.__cfBeacon=T}if(g&&T&&T.token){var P,R,B,O=!1,_=0;document.addEventListener("visibilitychange",function(){if("hidden"===document.visibilityState){if(x&&q()){var n=e();(null===B||void 0===B?void 0:B.url)==n&&null!==B&&void 0!==B&&B.triggered||M(),H(n)}!O&&B&&(O=!0,V())}else"visible"===document.visibilityState&&(_=(new Date).getTime())});var A={},I=function(e){if(!e||0===e.length)return null;var n=e.reduce(function(e,n){return e&&e.value>n.value?e:n});if(n&&n.sources&&n.sources.length){var t=n.sources.reduce(function(e,n){return e.node&&e.previousRect.width*e.previousRect.height>n.previousRect.width*n.previousRect.height?e:n});if(t)return t}},F=function(e){return e&&0!==e.length?e[e.length-1]:null},N=function(e){if(!e)return"";var n=e.localName;return e.id&&e.id.length>0&&(n+="#"+e.id),e.className&&e.className.length>0&&(n+="."+e.className.split(" ").join(".")),n},k=function(e){var n=window.location.pathname,t=F(e.entries);switch(A[e.name.toLowerCase()]={value:e.value,path:n},e.name){case"CLS":(t=I(e.entries))&&A.cls&&(A.cls.element=N(t.node),A.cls.currentRect=t.currentRect,A.cls.previousRect=t.previousRect);break;case"FID":t&&A.fid&&(A.fid.element=N(t.target),A.fid.name=t.name);break;case"LCP":t&&A.lcp&&(A.lcp.element=N(t.element),A.lcp.size=t.size,A.lcp.url=t.url)}};"function"==typeof PerformanceObserver&&((0,a.onLCP)(k),(0,a.onFID)(k),(0,a.onFCP)(k),(0,a.onINP)(k),(0,a.onTTFB)(k),PerformanceObserver.supportedEntryTypes&&PerformanceObserver.supportedEntryTypes.includes("layout-shift")&&(0,a.onCLS)(k));var x=T&&(void 0===T.spa||!0===T.spa),j=T.send&&T.send.to?T.send.to:void 0===T.version?"https://cloudflareinsights.com/cdn-cgi/rum":null,M=function(e){var n=function(e,n){t.resources=e,0!=n&&(t.bypassTiming=!0),T&&(1===T.r&&(t.resources=[]),(0,o.sendObjectBeacon)("",t,function(){},!1,j),void 0!==T.forward&&void 0!==T.forward.url&&(0,o.sendObjectBeacon)("",t,function(){},!1,T.forward.url))},t=v(e);if(t&&T){var r=t.tempResources;if(delete t.tempResources,x&&r&&0===r.length&&n([],0),!r)return;r.forEach(function(e,t){n(e,t)})}},V=function(){var e=p();x||(e.resources=[],delete e.tempResources),T&&(0,o.sendObjectBeacon)("",e,function(){},!0,j)},D=function(){var n=window.__cfRl&&window.__cfRl.done||window.__cfQR&&window.__cfQR.done;n?n.then(M):M(),B={id:h,url:e(),ts:(new Date).getTime(),triggered:!0}};"complete"===window.document.readyState?D():window.addEventListener("load",function(){window.setTimeout(D)});var q=function(){return x&&0===w.filter(function(e){return e.id===h}).length},H=function(e){w.push({id:h,url:e,ts:(new Date).getTime()}),w.length>3&&w.shift()};x&&(R=e(),function(n){var t=n.pushState;if(t){var r=function(){h=c(),"function"==typeof g.clearResourceTimings&&g.clearResourceTimings(),_=0};n.pushState=function(i,o,a){P=e(a);var c=e(),u=!0;return P==c&&(u=!1),u&&(q()&&((null===B||void 0===B?void 0:B.url)==c&&null!==B&&void 0!==B&&B.triggered||M(c),H(c)),r()),t.apply(n,[i,o,a])},window.addEventListener("popstate",function(n){q()&&((null===B||void 0===B?void 0:B.url)==P&&null!==B&&void 0!==B&&B.triggered||M(P),H(P)),P=e(),r()})}}(window.history))}}}()}()},function(e,n,t){"use strict";n.__esModule=!0,n.EventType=void 0;!function(e){e[e.Load=1]="Load",e[e.Additional=2]="Additional",e[e.WebVitalsV2=3]="WebVitalsV2"}(n.EventType||(n.EventType={}))},function(e,n,t){"use strict";function r(e,n,t,r,i){void 0===r&&(r=!1),void 0===i&&(i=null);var o=i||(n.siteToken&&n.versions.fl?"/cdn-cgi/rum?"+e:"/cdn-cgi/beacon/performance?"+e),a=!0;if(navigator&&"string"==typeof navigator.userAgent)try{var c=navigator.userAgent.match(/Chrome\/([0-9]+)/);c&&c[0].toLowerCase().indexOf("chrome")>-1&&parseInt(c[1])<81&&(a=!1)}catch(e){}if(navigator&&"function"==typeof navigator.sendBeacon&&a&&r){n.st=1;var u=JSON.stringify(n),s={type:"application/json"};navigator.sendBeacon(o,new Blob([u],s))}else{n.st=2;var u=JSON.stringify(n),f=new XMLHttpRequest;t&&(f.onreadystatechange=function(){4==this.readyState&&204==this.status&&t()}),f.open("POST",o,!0),f.setRequestHeader("content-type","application/json"),f.send(u)}}n.__esModule=!0,n.sendObjectBeacon=void 0,n.sendObjectBeacon=r},function(e,n,t){"use strict";n.__esModule=!0,n.onTTFB=n.onLCP=n.onINP=n.onFID=n.onFCP=n.onCLS=n.getTTFB=n.getLCP=n.getINP=n.getFID=n.getFCP=n.getCLS=void 0;var r,i,o,a,c,u=-1,s=function(e){addEventListener("pageshow",function(n){n.persisted&&(u=n.timeStamp,e(n))},!0)},f=function(){return window.performance&&performance.getEntriesByType&&performance.getEntriesByType("navigation")[0]},d=function(){var e=f();return e&&e.activationStart||0},l=function(e,n){var t=f(),r="navigate";return u>=0?r="back-forward-cache":t&&(r=document.prerendering||d()>0?"prerender":t.type.replace(/_/g,"-")),{name:e,value:void 0===n?-1:n,rating:"good",delta:0,entries:[],id:"v3-".concat(Date.now(),"-").concat(Math.floor(8999999999999*Math.random())+1e12),navigationType:r}},p=function(e,n,t){try{if(PerformanceObserver.supportedEntryTypes.includes(e)){var r=new PerformanceObserver(function(e){n(e.getEntries())});return r.observe(Object.assign({type:e,buffered:!0},t||{})),r}}catch(e){}},v=function(e,n){var t=function t(r){"pagehide"!==r.type&&"hidden"!==document.visibilityState||(e(r),n&&(removeEventListener("visibilitychange",t,!0),removeEventListener("pagehide",t,!0)))};addEventListener("visibilitychange",t,!0),addEventListener("pagehide",t,!0)},m=function(e,n,t,r){var i,o;return function(a){n.value>=0&&(a||r)&&((o=n.value-(i||0))||void 0===i)&&(i=n.value,n.delta=o,n.rating=function(e,n){return e>n[1]?"poor":e>n[0]?"needs-improvement":"good"}(n.value,t),e(n))}},g=-1,y=function(){return"hidden"!==document.visibilityState||document.prerendering?1/0:0},h=function(){v(function(e){var n=e.timeStamp;g=n},!0)},w=function(){return g<0&&(g=y(),h(),s(function(){setTimeout(function(){g=y(),h()},0)})),{get firstHiddenTime(){return g}}},T=function(e,n){n=n||{};var t,r=[1800,3e3],i=w(),o=l("FCP"),a=function(e){e.forEach(function(e){"first-contentful-paint"===e.name&&(u&&u.disconnect(),e.startTime<i.firstHiddenTime&&(o.value=e.startTime-d(),o.entries.push(e),t(!0)))})},c=window.performance&&window.performance.getEntriesByName&&window.performance.getEntriesByName("first-contentful-paint")[0],u=c?null:p("paint",a);(c||u)&&(t=m(e,o,r,n.reportAllChanges),c&&a([c]),s(function(i){o=l("FCP"),t=m(e,o,r,n.reportAllChanges),requestAnimationFrame(function(){requestAnimationFrame(function(){o.value=performance.now()-i.timeStamp,t(!0)})})}))},E=!1,S=-1,b=function(e,n){n=n||{};var t=[.1,.25];E||(T(function(e){S=e.value}),E=!0);var r,i=function(n){S>-1&&e(n)},o=l("CLS",0),a=0,c=[],u=function(e){e.forEach(function(e){if(!e.hadRecentInput){var n=c[0],t=c[c.length-1];a&&e.startTime-t.startTime<1e3&&e.startTime-n.startTime<5e3?(a+=e.value,c.push(e)):(a=e.value,c=[e]),a>o.value&&(o.value=a,o.entries=c,r())}})},f=p("layout-shift",u);f&&(r=m(i,o,t,n.reportAllChanges),v(function(){u(f.takeRecords()),r(!0)}),s(function(){a=0,S=-1,o=l("CLS",0),r=m(i,o,t,n.reportAllChanges)}))},C={passive:!0,capture:!0},L=new Date,P=function(e,n){r||(r=n,i=e,o=new Date,O(removeEventListener),R())},R=function(){if(i>=0&&i<o-L){var e={entryType:"first-input",name:r.type,target:r.target,cancelable:r.cancelable,startTime:r.timeStamp,processingStart:r.timeStamp+i};a.forEach(function(n){n(e)}),a=[]}},B=function(e){if(e.cancelable){var n=(e.timeStamp>1e12?new Date:performance.now())-e.timeStamp;"pointerdown"==e.type?function(e,n){var t=function(){P(e,n),i()},r=function(){i()},i=function(){removeEventListener("pointerup",t,C),removeEventListener("pointercancel",r,C)};addEventListener("pointerup",t,C),addEventListener("pointercancel",r,C)}(n,e):P(n,e)}},O=function(e){["mousedown","keydown","touchstart","pointerdown"].forEach(function(n){return e(n,B,C)})},_=function(e,n){n=n||{};var t,o=[100,300],c=w(),u=l("FID"),f=function(e){e.startTime<c.firstHiddenTime&&(u.value=e.processingStart-e.startTime,u.entries.push(e),t(!0))},d=function(e){e.forEach(f)},g=p("first-input",d);t=m(e,u,o,n.reportAllChanges),g&&v(function(){d(g.takeRecords()),g.disconnect()},!0),g&&s(function(){var c;u=l("FID"),t=m(e,u,o,n.reportAllChanges),a=[],i=-1,r=null,O(addEventListener),c=f,a.push(c),R()})},A=0,I=1/0,F=0,N=function(e){e.forEach(function(e){e.interactionId&&(I=Math.min(I,e.interactionId),F=Math.max(F,e.interactionId),A=F?(F-I)/7+1:0)})},k=function(){return c?A:performance.interactionCount||0},x=function(){"interactionCount"in performance||c||(c=p("event",N,{type:"event",buffered:!0,durationThreshold:0}))},j=0,M=function(){return k()-j},V=[],D={},q=function(e){var n=V[V.length-1],t=D[e.interactionId];if(t||V.length<10||e.duration>n.latency){if(t)t.entries.push(e),t.latency=Math.max(t.latency,e.duration);else{var r={id:e.interactionId,latency:e.duration,entries:[e]};D[r.id]=r,V.push(r)}V.sort(function(e,n){return n.latency-e.latency}),V.splice(10).forEach(function(e){delete D[e.id]})}},H=function(e,n){n=n||{};var t=[200,500];x();var r,i=l("INP"),o=function(e){e.forEach(function(e){e.interactionId&&q(e),"first-input"===e.entryType&&!V.some(function(n){return n.entries.some(function(n){return e.duration===n.duration&&e.startTime===n.startTime})})&&q(e)});var n,t=(n=Math.min(V.length-1,Math.floor(M()/50)),V[n]);t&&t.latency!==i.value&&(i.value=t.latency,i.entries=t.entries,r())},a=p("event",o,{durationThreshold:n.durationThreshold||40});r=m(e,i,t,n.reportAllChanges),a&&(a.observe({type:"first-input",buffered:!0}),v(function(){o(a.takeRecords()),i.value<0&&M()>0&&(i.value=0,i.entries=[]),r(!0)}),s(function(){V=[],j=k(),i=l("INP"),r=m(e,i,t,n.reportAllChanges)}))},J={},z=function(e,n){n=n||{};var t,r=[2500,4e3],i=w(),o=l("LCP"),a=function(e){var n=e[e.length-1];if(n){var r=n.startTime-d();r<i.firstHiddenTime&&(o.value=r,o.entries=[n],t())}},c=p("largest-contentful-paint",a);if(c){t=m(e,o,r,n.reportAllChanges);var u=function(){J[o.id]||(a(c.takeRecords()),c.disconnect(),J[o.id]=!0,t(!0))};["keydown","click"].forEach(function(e){addEventListener(e,u,{once:!0,capture:!0})}),v(u,!0),s(function(i){o=l("LCP"),t=m(e,o,r,n.reportAllChanges),requestAnimationFrame(function(){requestAnimationFrame(function(){o.value=performance.now()-i.timeStamp,J[o.id]=!0,t(!0)})})})}},U=function e(n){document.prerendering?addEventListener("prerenderingchange",function(){return e(n)},!0):"complete"!==document.readyState?addEventListener("load",function(){return e(n)},!0):setTimeout(n,0)},W=function(e,n){n=n||{};var t=[800,1800],r=l("TTFB"),i=m(e,r,t,n.reportAllChanges);U(function(){var o=f();if(o){if(r.value=Math.max(o.responseStart-d(),0),r.value<0||r.value>performance.now())return;r.entries=[o],i(!0),s(function(){r=l("TTFB",0),(i=m(e,r,t,n.reportAllChanges))(!0)})}})};n.getFCP=T,n.onFCP=T,n.getCLS=b,n.onCLS=b,n.getFID=_,n.onFID=_,n.getINP=H,n.onINP=H,n.getLCP=z,n.onLCP=z,n.getTTFB=W,n.onTTFB=W},function(e,n,t){"use strict";function r(e,n,t){var r=n&&t||0;"string"==typeof e&&(n="binary"===e?new Array(16):null,e=null),e=e||{};var a=e.random||(e.rng||i)();if(a[6]=15&a[6]|64,a[8]=63&a[8]|128,n)for(var c=0;c<16;++c)n[r+c]=a[c];return n||o(a)}var i=t(5),o=t(6);e.exports=r},function(e,n,t){"use strict";var r="undefined"!=typeof crypto&&crypto.getRandomValues&&crypto.getRandomValues.bind(crypto)||"undefined"!=typeof msCrypto&&"function"==typeof window.msCrypto.getRandomValues&&msCrypto.getRandomValues.bind(msCrypto);if(r){var i=new Uint8Array(16);e.exports=function(){return r(i),i}}else{var o=new Array(16);e.exports=function(){for(var e,n=0;n<16;n++)0==(3&n)&&(e=4294967296*Math.random()),o[n]=e>>>((3&n)<<3)&255;return o}}},function(e,n,t){"use strict";function r(e,n){var t=n||0,r=i;return[r[e[t++]],r[e[t++]],r[e[t++]],r[e[t++]],"-",r[e[t++]],r[e[t++]],"-",r[e[t++]],r[e[t++]],"-",r[e[t++]],r[e[t++]],"-",r[e[t++]],r[e[t++]],r[e[t++]],r[e[t++]],r[e[t++]],r[e[t++]]].join("")}for(var i=[],o=0;o<256;++o)i[o]=(o+256).toString(16).substr(1);e.exports=r}]);

==> infinite_lower_b.tex <==
%\subsection{Lower bound}
%
%\begin{theorem}\label{thm:infinite-lwoer-bound}
%Given any $S$, $\gamma \in[\frac{1}{2},1)$, $\varepsilon \leq \frac{1}{56(1-\gamma)}$, and $\Cstar \geq \frac{2}{S}$. There exists some MDP class $\mathsf{MDP}(\Cstar) = \big\{\mathcal{M} = (\mathcal{S}, \mathcal{A}, P, r, \gamma)\big\}$ with some initial state distribution $\rho$ and behavior policy $\pi_{\mathsf{b}}$, such that 
%\begin{align*}
%\max_{(s, a) \in \cS \times \cA}\frac{\min\big\{d^{\star}(s, a), \frac{1}{S}\big\}}{\myrho(s, a)} = \Cstar
%\end{align*}
%In addition, 
%\begin{align*}
%\inf_{\pi}\sup_{\mathcal{M} \in \mathsf{MDP}(\Cstar)} \mathbb{E}_{\mathcal{M}}\big[\langle \rho, V^{\star} - V^{\pi}\rangle \big] \ge \min \left( c_1 \sqrt{\frac{ \Cstar S}{(1-\gamma)^3 N}}, \frac{1}{1-\gamma} \right),
%\end{align*}
%for some small enough constant $c_1$.
%% provided that
%% \begin{align*}
%% N \lesssim \frac{\Cstar S}{(1-\gamma)^3\varepsilon^2}.
%% \end{align*}
%\end{theorem}
%\begin{proof}
%See Appendix~\ref{proof:thm-infinite-lb}.
%\end{proof}


==> infinite_markov.tex <==
\section{Discounted infinite-horizon MDPs with Markovian data}
\label{sec:main-infinite-markov}

In this section, we extend the i.i.d.~sampling model \eqref{eq:sampling-offline-inf-iid} for discounted infinite-horizon MDPs to accommodate Markovian data. 


\subsection{Sampling models and assumptions}
\label{sec:models-infinite-markov}

 

\paragraph{A single Markovian trajectory.}  Suppose that we have access to a historical dataset $\mathcal{D}$, which comprises a single trajectory of samples with length $T$ generated by a behavior policy $\pib$. More precisely, the sample trajectory starts from an arbitrary state $s_0$ and takes the form
%
\begin{align}
	\{s_0, a_0, s_1, a_1,\cdots, s_T, a_T\}, 
	\label{eq:data-Markovian}
\end{align}
%
which is generated by the MDP $\mathcal{M}$ (cf.~Section~\ref{sec:models-infinite}) in the following manner 
%
\begin{align}
	a_t \sim \pib(\cdot \mymid s_t), \qquad  s_t' = s_{t+1} \sim P(\cdot \mymid s_t, a_t), \qquad\quad  0\leq t \leq T.
\end{align}
%
Note that the dataset $\mathcal{D}$ here consists of a single trajectory, thus resulting in substantially more complicated statistical dependency in comparison to the independent sampling model. 
This model has also been investigated in our companion paper \citet{yan2022efficacy}, although the focus therein is on model-free algorithms. 
With regards to the Markov chain generating the above sample trajectory, 
we shall assume it to be uniformly ergodic (see, e.g., \citet[Definition 1.1]{paulin2015concentration}). We denote by $\mub$ the stationary state-action distribution of this chain, 
and let $\tmix$ indicate its mixing time as follows \citep{paulin2015concentration}
%
\begin{subequations}
\begin{align}
	\tmix(\delta) &\coloneqq \min \left\{ t \,\,\Big|\, 
	\max_{s_0 \in \cS } d_{\mathsf{TV}}\big( \mu(s_t, a_t \mymid s_0) , \mub \big) \leq \delta \right\}, \label{eq:defn-mixing-time-delta} \\
	\tmix &\coloneqq \tmix(1/4),  \label{eq:defn-mixing-time}
\end{align}
\end{subequations} 
%
where $\mu(s_t, a_t \mymid s_0)$ denotes the probability distribution of $(s_t,a_t)$ given the initial state $s_0$, 
and $d_{\mathsf{TV}}(\mu,\nu)$ indicates the total-variation distance between two distributions $\mu$ and $\nu$. 


Similar to Definition~\ref{assumption:concentrate-infinite}, we introduce the following concentrability to capture the distribution shift. 
%
% the key concentrability for the infinite-horizon case which is weaker than the assumption in \citep{rashidinejad2021bridging}:
%
\begin{definition}[Single-policy clipped concentrability for discounted infinite-horizon MDPs] 
\label{assumption:concentrate-infinite-markov}
%
The single-policy clipped concentrability coefficient of the  dataset $\mathcal{D}$ (cf.~\eqref{eq:data-Markovian}) is given by
%
\begin{align}
	\Cstar \coloneqq \max_{(s, a) \in \cS \times \cA}\frac{\min\big\{d^{\star}(s, a), \frac{1}{S}\big\}}{\mub(s, a)} .
	\label{eq:concentrate-infinite-markov}
\end{align}
%
%. In this paper, we take $\Cstar$ as the smallest quantity satisfying \eqref{eq:concentrate-infinite}, and refer to it as the single-policy clipped concentrability coefficient. 
\end{definition}
%
In comparison to Definition~\ref{assumption:concentrate-infinite}, the denominator in \eqref{eq:concentrate-infinite-markov} uses the stationary distribution $\mub$ of the underlying Markov chain. 
In particular, if the initial state $s_0$ is also drawn from this distribution $\mub$, then it is self-evident that $d^{\pib}=\mub$; in such a case, Condition~\eqref{eq:concentrate-infinite-markov} can be alternatively expressed as
%
\begin{align}
	\Cstar  = \max_{(s, a) \in \cS \times \cA}\frac{\min\big\{d^{\star}(s, a), \frac{1}{S}\big\}}{d^{\pib}(s, a)}  ,
	\label{eq:concentrate-infinite-alternative-markov}
\end{align}
%
which is largely dictated by the closeness between the resulting occupancy of the target policy $\pi^{\star}$ and that of the behavior policy $\pib$.  


 


\subsection{A subsampling trick}
\label{sec:sample-split-infinite-markov}


Before continuing, we single out a crucial property that allows us to reuse the algorithmic idea developed for the i.i.d.~sampling model. 
Imagine that the Markovian trajectory runs until $t=\infty$, although only the first $T$ sample transitions are revealed to us. 
For any given $(s,a)$,  denote by $t_i(s, a)$ the time stamp when the trajectory visits this state-action pair $(s, a)$ for the $i$-th time.
As has been rigorized in  \citet[Section B.1]{li2021sample}, for any given $(s,a)\in \cS\times \cA$, the following sample transitions 
%
\begin{align}
	\left\{(s, a, s_{t_i(s, a)+1}) \mid  1\leq  i \leq T\right\}
\end{align}
%
are statistically independent, resembling the i.i.d.~sampling model in some sense.


% In view of this observation, we can pick first $N(s, a)$ transitions for each state-action pair $(s, a)$ to get independent samples.

% Given any fixed integer $N(s,a)$ for every state-action $(s, a) \in \cS \times \cA$, suppose we have access to some lower bound $\Ntrim(s, a)$ on $N(s, a)$.
% Employ the first $\Ntrim(s, a)$ transitions to construct an empirical transition kernel $\widehat{P}$.
% By construction, $\{\widehat{P}_{s, a}\}$ are independent of each other.
On a high level, our algorithm is built upon a two-fold subsampling trick to decouple the statistical dependence across the sample rollout. 
Roughly speaking, the main steps are as follows, with a detailed description provided in Algorithm~\ref{alg:vi-lcb-infinite-split-markov}. 
%
\begin{itemize}
	\item[i)] Split data into two parts: $\Dmain$ and $\Daux$, each containing half of the sample trajectory. Let $\Nmain(s, a)$ denote the number of sample transitions in $\Dmain$ from state $s$ when action $a$ is taken.

	\item[ii)] For each $(s, a) \in \cS\times\cA$, use $\Daux$ to compute lower bounds $\{\Ntrim(s, a)\}$ on $\{\Nmain(s, a)\}$. Subsample the first $\Ntrim(s, a)$ sample transitions from $\Dmain$ to construct data subset $\Dtrim$. 

	\item[iii)] Run VI-LCB (i.e., Algorithm~\ref{alg:vi-lcb-infinite}) on the subsampled dataset $\Dtrim$.
\end{itemize}


\begin{algorithm}[h]
\DontPrintSemicolon
	\textbf{input:} Markovian dataset $\mathcal{D}$ (cf.~\eqref{eq:data-Markovian}); reward function $r$. \\

	\textbf{subsampling:} run the following procedure to generate the subsampled dataset $\Dtrim$. 
	{ \begin{itemize}
	\item[1)] {\em Data splitting.} Split $\mathcal{D}$ into two halves:  $\Dmain = \{s_0, a_0, s_1, a_1,\cdots, s_{T/2}\}$ (which contains the first $T/2$ transitions), and $\Daux = \{s_{T/2}, a_{T/2}, s_{T/2+1}, a_{T/2+1},\cdots, s_{T}\}$ (which contains the remaining $T/2$ transitions);    we let $\Nmain(s, a)$ (resp.~$\Naux(s, a)$) denote the number of sample transitions in $\Dmain$ (resp.~$\Daux$) that transition from state $s$ with action $a$ taken.  

	\item[2)] {\em Lower bounding $\{\Nmain(s, a)\}$ using $\Daux$.} For each $(s,a)\in \cS\times\cA$, let 
	\begin{align}
	\Ntrim_k(s, a) \coloneqq \frac{1}{3}\Naux(s, a)\mathds{1}\Big(\Naux(s, a) > k\log\frac{SA}{\delta}\Big),
		\qquad k\in \mathbb{N}.
	\label{eq:defn-Ntrim-infinite}
\end{align}
			If we know $\tmix$, set $\Ntrim(s, a) = \Ntrim_{665\tmix}(s, a)$; otherwise, set $\Ntrim(s, a) = \Ntrim_{\widehat{k}(s,a)}(s, a)$ with
\begin{align}\label{eq:defn-k-hat-infinite}
	\widehat{k}(s,a) = \min\big\{k : \Ntrim_{k}(s, a) \le \Nmain(s, a) \big\}.
\end{align} 

	\item[3)] {\em Subsampling.} Let ${\Dmain}'$ be the set of all sample transitions (i.e., the tuples taking the form $(s,a,s')$) from $\Dmain$. 
		Subsample ${\Dmain}'$ to obtain $\Dtrim$, such that for each $(s,a)\in \cS\times \cA$, $\Dtrim$ contains the first $\Ntrim(s, a)$ sample transitions from ${\Dmain}'$. 
\end{itemize}
}

	\textbf{run VI-LCB:} set $\mathcal{D}_0 = \Dtrim$, and run Algorithm~\ref{alg:vi-lcb-infinite} to compute a policy $\widehat{\pi}$.  
	\caption{Subsampled VI-LCB for discounted infinite MDPs with Markovian data}
 	\label{alg:vi-lcb-infinite-split-markov}
\end{algorithm}




The lemma below states several properties about $\Ntrim_{k}(s, a)$ that resemble the properties in Lemma~\ref{lemma:Ntrim-LB}. 
%
\begin{lemma} \label{lem:sample-split-infinite-markov}
With probability at least $1-2\delta$, the quantities constructed in \eqref{eq:defn-Ntrim-infinite} obey
%
\begin{subequations}
\label{eq:samples-infinite-markov}
\begin{align}
	\Ntrim_{k}(s, a)  &\le \Nmain(s, a),  &&\text{for all }k \ge 665t_{\mathsf{mix}} \label{eq:samples-infinite-UB-markov}\\
%
	\max\bigg\{\Ntrim_{k}(s, a), 222t_{\mathsf{mix}}\log\frac{SA}{\delta}\bigg\} &\ge \frac{ T\mub(s, a) }{12},\qquad &&\text{for all }k \le 665t_{\mathsf{mix}} 
	\label{eq:samples-infinite-LB-markov}
%	
\end{align}
\end{subequations}
%
simultaneously for all $(s, a) \in \cS \times \cA$. 
\end{lemma}
%
Lemma~\ref{lem:sample-split-infinite-markov} tells us the following important properties: 
%
\begin{itemize}
	\item When $\Ntrim(s, a) = \Ntrim_{665\tmix}(s, a)$, then it follows directly from Lemma~\ref{lem:sample-split-infinite-markov} that
	%
\begin{subequations}
\label{eq:samples-infinite-markov-with-tmix}
\begin{align}
	\label{eq:samples-infinite-markov-know-tmix}
	%\Ntrim(s, a)  &\le \Nmain(s, a),   \qquad 
%
	\max\bigg\{\Ntrim(s, a), 222t_{\mathsf{mix}}\log\frac{SA}{\delta}\bigg\} \ge \frac{ T\mub(s, a) }{12}. 
\end{align}
%	

	\item When $\Ntrim(s, a) = \Ntrim_{\widehat{k}(s,a)}(s, a)$ (cf.~\eqref{eq:defn-k-hat-infinite}), it is easy to show that $\widehat{k}(s,a) \leq 665\tmix$ and 
	%
\begin{align}
	\label{eq:samples-infinite-markov-no-tmix}
	\max\bigg\{\Ntrim(s, a), 222t_{\mathsf{mix}}\log\frac{SA}{\delta}\bigg\} \ge \frac{ T\mub(s, a) }{12}. 
\end{align}
%
	To see why this is true, it suffices to combine the fact \eqref{eq:samples-infinite-UB-markov} with the choice \eqref{eq:defn-k-hat-infinite}.   
\end{subequations}

\end{itemize}


\begin{proof}[Proof of Lemma~\ref{lem:sample-split-infinite-markov}]
Since $\Ntrim_{k}(s, a)$ is non-increasing as $k$ grows, it is sufficient to prove~\eqref{eq:samples-infinite-markov} for $k = 665t_{\mathsf{mix}}$.
Repeating similar arguments as for  \citet[Lemma 8]{li2021sample}  --- which concerns the concentration of measure for the empirical distribution of a uniformly ergodic Markov chain --- implies that: with probability at least $1-\delta$,
\begin{subequations}
\label{eqn:naux-cases}
\begin{align}
\label{eqn:naux-conct}
\bigg|\Naux(s, a) - \frac{T\mub(s, a)}{2}\bigg| \le \frac{T\mub(s, a)}{4}
\end{align}
holds for all $(s,a)$ obeying $\frac{T\mub(s, a)}{2} \ge 443t_{\mathsf{mix}}\log\frac{SA}{\delta}$, and
\begin{align}
\Naux(s, a) \le 665t_{\mathsf{mix}}\log\frac{SA}{\delta}
\end{align}
\end{subequations}
	holds for all $(s,a)$ obeying $\frac{T\mub(s, a)}{2} < 443t_{\mathsf{mix}}\log\frac{SA}{\delta}$; we omit the proof for brevity.
Recalling the definition \eqref{eq:defn-Ntrim-infinite}, 
we can readily see from \eqref{eqn:naux-cases} that when $k = 665t_{\mathsf{mix}}$:   $\Ntrim_{k}(s, a) = 0$  if $\frac{T\mub(s, a)}{2} < 443t_{\mathsf{mix}}\log\frac{SA}{\delta}$, and 
\begin{align}
\frac{T\mub(s, a)}{12} \le \Ntrim_{k}(s, a) \le \frac{T\mub(s, a)}{4}
\label{eqn:naux-cases-2}
\end{align}
% 
if $\frac{T\mub(s, a)}{2} > 1330t_{\mathsf{mix}}\log\frac{SA}{\delta}$. Therefore, we have established \eqref{eq:samples-infinite-LB-markov}.

We then prove relation~\eqref{eq:samples-infinite-UB-markov}. Similar to \eqref{eqn:naux-conct}, with probability at least $1-\delta$ we have
\begin{align}\label{eqn:Nmain-case}
\bigg|\Nmain(s, a) - \frac{T\mub(s, a)}{2}\bigg| \le \frac{T\mub(s, a)}{4}
\end{align}
	for all $(s,a)$ with $\frac{T\mub(s, a)}{2} \ge 443t_{\mathsf{mix}}\log\frac{SA}{\delta}$. 
Putting \eqref{eqn:naux-cases-2} and \eqref{eqn:Nmain-case} together establishes relation~\eqref{eq:samples-infinite-UB-markov}. 
\end{proof}




%\begin{remark}
%\label{remark:union} 
%	\yxc{check later} 
%Rigorously speaking, $\big\{\Ntrim_{\widehat{k}}(s, a)\big\}$ in Algorithm~\ref{alg:vi-lcb-infinite-split-markov} in fact, depends on data set $\Dmain$ through $s_{T/2}$ and $\widehat{k}$.
%To deal with this issue, we can take union bound over any $(s_{T/2}, \widehat{k}) = (s, k) \in \cS \times [665\tmix]$.
%\end{remark}




\subsection{Performance guarantees}

We are now ready to present our theoretical guarantees for Algorithm~\ref{alg:vi-lcb-infinite-split-markov} in the presence of Markovian data. 

\begin{theorem} \label{thm:infinite-markov}
%
Consider any  $\gamma \in [\frac{1}{2},1)$, $0<\delta <1$ and any $ \varepsilon \in \big(0, \frac{1}{1-\gamma} \big]$. 
Suppose that the number of iterations exceeds $\taumax > \frac{1}{1-\gamma}\log\frac{T}{1-\gamma}$. 
With probability at least $1-3\delta,$  the policy $\widehat{\pi}$ returned by Algorithm~\ref{alg:vi-lcb-infinite-split-markov} obeys
%
\begin{align}
	V^{\star}(\rho) - V^{\widehat{\pi}}(\rho) \leq \varepsilon,
\end{align}
as long as the penalty terms are chosen according to the Bernstein-style quantity \eqref{def:bonus-Bernstein-infinite} for any constant 
$\cb \ge 144$, and the total number of samples exceeds 
%
\begin{align}
T\geq\frac{c_1 S\Cstar \log\frac{665S\tmix T }{(1-\gamma)\delta}}{(1-\gamma)^{3}\varepsilon^{2}} + \frac{c_1\tmix S\Cstar \log\frac{665S\tmix T }{(1-\gamma)\delta}}{(1-\gamma)^{2}\varepsilon}
	\label{eq:sample-complexity-infinit-markov}
\end{align}
	for some large enough numerical constant $c_{1} >0$ (e.g., $c_1 = 22000$). 
%
%Here, $c_1>0$ is some sufficiently large constant.
\end{theorem}

Theorem~\ref{thm:infinite-markov} provides a sample complexity bound that is very similar to the i.i.d.~sampling case (i.e., Theorem~\ref{thm:infinite}), 
except that the length $T$ of the sample trajectory also needs to exceed some linear scaling in the mixing time. 
This is unavoidable though (see also other related works \citet{yan2022efficacy,li2021sample}); unless the sample trajectory mixes well, in general one would not be able to obtain enough information associated with all states given only this sample trajectory. 
In comparison to the variance-reduced offline model-free algorithm proposed in  \citet{yan2022efficacy}, 
our sample complexity \eqref{eq:sample-complexity-infinit-markov} is strictly better (more precisely, the sample complexity in  \citet{yan2022efficacy} has two additional terms $\frac{SC^{\star}}{(1-\gamma)^4\varepsilon} + \frac{\tmix C^{\star}}{(1-\gamma)^3\varepsilon}$ and hence incurs a longer burn-in phase than the one derived herein). 


\begin{proof}[Proof of Theorem~\ref{thm:infinite-markov}]
	The proof follows very similar arguments as for Theorem~\ref{thm:Bernstein-auxiliary-infinite},  although we need to replace Lemma~\ref{lem:sample-split-infinite} by Lemma~\ref{lem:sample-split-infinite-markov}.
For brevity, we shall only point out the parts of the analysis that need modification. 


To begin with, we shall suppose for the moment that 
%
\[
	N(s,a)=\Ntrim(s,a)=\Ntrim_k(s,a),\qquad \forall (s,a)\in \cS\times \cA
\]
%
for a fixed integer $k\leq 665\tmix$, and assume that the two parts $\Daux$ and $\Dmain$ are statistically independent.  We will come back to remove these two assumptions towards the end of this proof.   




This analysis mainly differs from that of Theorem~\ref{thm:Bernstein-auxiliary-infinite} in its Step 4 when controlling $\langle d^\star, b^\star \rangle$, which we shall detail now.  
Let us first divide  $\cS$ into the following two disjoint state subsets:
%
\begin{subequations}
\label{eq:defn-Ssmall-Slarge-inf-markov}
%
\begin{align}
	\cS^{\mathsf{small}} \coloneqq \bigg\{ s\in \cS \mid  T\mub\big(s, \pi^{\star}(s) \big) \leq 2660\tmix \log \frac{SA}{\delta} \bigg\}; \label{eq:defn-Ssmall-inf-markov}\\
	\cS^{\mathsf{large}} \coloneqq \bigg\{ s\in \cS \mid  T\mub\big(s, \pi^{\star}(s) \big) > 2660\tmix \log \frac{SA}{\delta} \bigg\}. \label{eq:defn-Slarge-inf-markov}
\end{align}
%
\end{subequations}
%
\begin{itemize}
%
\item
Firstly, for any state $s \in \cS^{\mathsf{small}}$, combine Definition~\ref{assumption:concentrate-infinite-markov} with the definition of $\cS^{\mathsf{small}}$ to give 
%
\begin{align}
	\min \Big\{ d^{\star}(s) , \frac{1}{S} \Big\} 
	\le \Cstar  \mub \big(s, \pi^{\star}(s) \big) \le \frac{2660 \Cstar \tmix \log \frac{T}{(1-\gamma)\delta}}{T} < \frac{1}{S}, 
\end{align}
%
provided that $T > 2660S \Cstar \tmix \log \frac{T }{(1-\gamma)\delta}$. An immediate consequence of this result is that
%
%
\begin{align}
	 d^{\star}(s)  
	\le  \frac{2660 \Cstar \tmix \log \frac{T}{(1-\gamma)\delta}}{T} < \frac{1}{S}.  
\end{align}
%
Taking this inequality together with the fact below (see the definition \eqref{def:bonus-Bernstein-infinite}) 
%
\begin{align}
	b^{\star}(s) \coloneqq b\big(s, \pi^{\star}(s); \widehat{V} \big) \leq \frac{1}{1-\gamma} + \frac{5}{T},
\end{align}
%
we can demonstrate that 
%
\begin{align}
\sum_{s\in\cS^{\mathsf{small}}}	d^{\star}(s) b^{\star}(s) &\leq \sum_{s\in\cS^{\mathsf{small}}} \left( \frac{2660 \Cstar \tmix \log \frac{T}{(1-\gamma)\delta}}{(1-\gamma)T} +   d^{\star}(s) \frac{5}{T} \right) \leq  \frac{2660 S \Cstar \tmix \log \frac{T}{(1-\gamma)\delta}}{(1-\gamma)T} +  \frac{5}{T}. \label{eq:infinite-bernstein-small-result-markov}
\end{align}
%



\item Secondly, we look at any state $s \in \cS^{\mathsf{large}}$. From the definition \eqref{def:bonus-Bernstein-infinite} of $b(s,a;V) $, one obtains 
%
\begin{align}
	b^{\star}(s) 
	&\le \sqrt{\frac{\cb\log\frac{T }{(1-\gamma)\delta}}{N\big(s, \pi^{\star}(s)\big)}\mathsf{Var}_{\widehat{P}_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} +  \frac{2\cb\log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)N\big(s, \pi^{\star}(s)\big)} + \frac{5}{T}\notag\\
	& \overset{\mathrm{(i)}}{\le} \sqrt{\frac{\cb\log\frac{T  }{(1-\gamma)\delta}}{N\big(s, \pi^{\star}(s)\big)}\left(2\mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big) 
	+ \frac{41\log\frac{2T}{(1-\gamma)\delta}}{(1-\gamma)^2N\big(s, \pi^{\star}(s)\big)}\right)} + \frac{2\cb \log\frac{T }{(1-\gamma)\delta}}{(1-\gamma)N\big(s, \pi^{\star}(s)\big)}   +\frac{5}{T} \notag\\
	& \overset{\mathrm{(ii)}}{\le} \sqrt{\frac{2\cb\log\frac{T }{(1-\gamma)\delta}}{N\big(s, \pi^{\star}(s)\big)}\mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} +  \frac{4\cb\log\frac{T }{(1-\gamma)\delta}}{(1-\gamma)N\big(s, \pi^{\star}(s)\big)}, \label{eq:infinite-bernstein-large-result-middle-markov}
\end{align}
%
where (i) comes from Lemma~\ref{lem:Bernstein-infinite} and inequality~\eqref{eq:Vhar-Vstarhat-diff-1/T-inf}, (ii) follows since $\sqrt{x+y}\leq \sqrt{x}+\sqrt{y}$ for any $x,y\geq 0$ and $T \geq N(s,a)$ for $\cb$ large enough. Moreover, 
it is seen that
\begin{align}
	\frac{1}{N\big(s, \pi^{\star}(s)\big)} \overset{\mathrm{(i)}}{\le} \frac{12}{T\mub \big(s, \pi^{\star}(s)\big)} \overset{\mathrm{(ii)}}{\le} \frac{12\Cstar}{T \min\big\{d^{\star}(s), \frac{1}{S}\big\}} \leq \frac{12\Cstar}{T}\left(\frac{1}{d^{\star}(s)} + S\right), \label{eq:infinite-N-to-d-bound}
\end{align}
%
where (i) follows from \eqref{eq:samples-infinite-markov-with-tmix},
		  and (ii) invokes Definition~\ref{assumption:concentrate-infinite-markov}.
		Plugging this inequality into \eqref{eq:infinite-bernstein-large-result-middle-markov} gives 
%
\begin{align}
	b^{\star}(s) &\leq \sqrt{\frac{2\cb\log\frac{T  }{(1-\gamma)\delta}}{N\big(s, \pi^{\star}(s)\big)}\mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} +  \frac{4\cb\log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)N\big(s, \pi^{\star}(s)\big)} \notag\\
	&\leq \underset{\eqqcolon\, \alpha_1(s) }{\underbrace{ \sqrt{\frac{24\cb  \Cstar \log\frac{T }{(1-\gamma)\delta}}{T} \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)}\left(\frac{1}{\sqrt{d^{\star}(s)}} + \sqrt{S}\right) }} + \underset{\eqqcolon\, \alpha_2(s) }{\underbrace{ \frac{48\cb \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}\left(\frac{1}{d^{\star}(s)} + S\right) }}, \label{eq:infinite-bernstein-large-result-markov}
\end{align}
%
where the last line also applies the elementary inequality $\sqrt{x+y}\leq \sqrt{x}+\sqrt{y}$ for any $x,y\geq 0$.


To continue, observe that summing the first terms in \eqref{eq:infinite-bernstein-large-result-markov} over $s\in \cS^{\mathsf{large}}$ satisfies 
%
\begin{align}
	&\sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s) \alpha_1(s) \notag\\
	&\quad = \sqrt{\frac{24\cb \Cstar \log\frac{T  }{(1-\gamma)\delta}}{T} } \left( \sum_{s\in\cS^{\mathsf{large}}} \sqrt{d^{\star}(s)  \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} + \sum_{s\in\cS^{\mathsf{large}}}\sqrt{d^{\star}(s)} \sqrt{Sd^{\star}(s)\mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} \right)\notag\\
	&\quad \overset{\mathrm{(i)}}{\leq} \sqrt{\frac{24\cb \Cstar \log\frac{T  }{(1-\gamma)\delta}}{T} } 
	\Bigg( \sqrt{S}  \sqrt{\sum_{s\in\cS^{\mathsf{large}}}  d^{\star}(s)  \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)}  
	 + \sqrt{\sum_{s\in\cS^{\mathsf{large}}} d^{\star}(s) S\mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} \Bigg) \notag\\
	&\quad = \sqrt{\frac{96\cb S\Cstar \log\frac{T }{(1-\gamma)\delta}}{T} } \sqrt{\sum_{s\in\cS^{\mathsf{large}}} d^{\star}(s) \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)}, \label{eq:infinite-bernstein-large-result1-markov}
\end{align}
%
where (i) comes from  Cauchy-Schwarz and the fact $\sum_s d^{\star}(s)=1$. 
In addition, the sum of the second terms in \eqref{eq:infinite-bernstein-large-result-markov} over $s\in \cS^{\mathsf{large}}$ obeys
%
\begin{align}
	\sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s) \alpha_2(s)
	\leq \frac{96\cb S \Cstar \log\frac{T }{(1-\gamma)\delta}}{(1-\gamma)T}, \label{eq:infinite-bernstein-large-result2-markov}
\end{align}
%
which follows since $\sum_s d^{\star}(s)=1$. 
Combine \eqref{eq:infinite-bernstein-large-result1-markov} and \eqref{eq:infinite-bernstein-large-result2-markov} with \eqref{eq:infinite-bernstein-large-result-markov} to yield
%
\begin{align}
	& \sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s) b^{\star}\big(s, \pi^{\star}(s) \big)
		\leq \sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s) \alpha_1(s) + \sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s) \alpha_2(s)
\notag\\
	& \qquad \le \sqrt{\frac{96\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{T} } \sqrt{\sum_{s\in\cS^{\mathsf{large}}} d^{\star}(s) \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} + \frac{96\cb S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}. \label{eq:infinite-bernstein-large-result-all-markov}
\end{align}
% 
\end{itemize}


 The above results \eqref{eq:infinite-bernstein-small-result-markov} and \eqref{eq:infinite-bernstein-large-result-all-markov} taken collectively give
%
\begin{align*}
	& \big\langle d^{\star}, b^\star \big\rangle  
	=\sum_{s\in\cS^{\mathsf{large}}}d^{\star}(s)b^{\star}(s) + \sum_{s\in\cS^{\mathsf{small}}}d^{\star}(s)b^{\star}(s) \\
&\quad \leq \sqrt{\frac{96\cb S\Cstar \log\frac{T }{(1-\gamma)\delta}}{T} } \sqrt{\sum_{s\in\cS^{\mathsf{large}}} d^{\star}(s) \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} + \frac{96\cb  S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}\\
&\quad\qquad + \frac{2660 S\Cstar \tmix \log \frac{T }{(1-\gamma)\delta}}{(1-\gamma)T} + \frac{5}{T} \\
&\quad \overset{\mathrm{(i)}}{\leq} \sqrt{\frac{96\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{T} } \sqrt{\sum_{s\in\cS} d^{\star}(s) \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big)} + \frac{192\cb \tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}\\
&\quad \overset{\mathrm{(ii)}}{\leq} \frac{2}{\gamma}\sqrt{\frac{96\cb S\Cstar \log\frac{T }{(1-\gamma)\delta}}{(1-\gamma)T}  \big\langle d^{\star}, b^{\star}\big\rangle}  + \frac{1}{\gamma}\sqrt{\frac{192\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}  }+ \frac{192\cb\tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}, \notag \\
&\quad \overset{\mathrm{(iii)}}{\leq} 4\sqrt{\frac{96\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}  \big\langle d^{\star}, b^{\star}\big\rangle}  + 2\sqrt{\frac{192\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}  }+ \frac{192\cb\tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}, \notag \\
&\quad \overset{\mathrm{(iv)}}{\leq} \frac{1}{2} \big\langle d^{\star}, b^{\star}\big\rangle + \frac{768\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}  + \sqrt{\frac{768\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}  }+ \frac{192\cb \tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}. 
\end{align*}
%
Here, (i) follows when $\cb$ is sufficiently large, $\tmix\geq 1$ and $\Cstar \geq 1/S$ (see \eqref{eq:Cstar_lower_bound_infinite}), 
(ii) holds by recalling~\eqref{eq:sum-d-Var-UB-123-infinite} that  
%
\begin{align*}
	\sum_{s\in\cS} d^{\star}(s) \mathsf{Var}_{P_{s, \pi^{\star}(s)}}\big(\widehat{V}\big) 
	\le \frac{2}{\gamma^2(1-\gamma)} + \frac{4}{\gamma^2(1-\gamma)}\big\langle d^{\star}, b^{\star}\big\rangle; 
\end{align*}
%
(iii) is valid since $\gamma \in [\frac{1}{2}, 1)$, and (iv) follows since $2xy\leq x^2 + y^2$. Rearrange terms to yield
%
\begin{align*}
	\big\langle d^{\star}, b^{\star} \big\rangle & \leq \sqrt{\frac{3072\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T}} + \frac{1920\cb \tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)T},
\end{align*}
%
which in turn leads to 
\begin{align}
	\big\langle \rho, V^{\star} - V^{\widehat{\pi}}\big\rangle 
	\leq \frac{2\big\langle d^{\star}, b^{\star} \big\rangle}{1-\gamma} \leq 120\sqrt{\frac{\cb S\Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)^3T}} + \frac{3840\cb \tmix S \Cstar \log\frac{T  }{(1-\gamma)\delta}}{(1-\gamma)^2T},
\end{align}
where the first inequality follows from relation~\eqref{eqn:brahms-reduction}. 


% For any accuracy level $\varepsilon$, 


Finally, we explain how to relax  the two strong assumptions imposed at the beginning of this proof.  
%
\begin{itemize}
	\item Note that when $\tmix$ is not known {\em a priori}, the choice $\widehat{k}(s,a)$ is not a fixed integer independent from the data. 
		Fortunately, we have already demonstrated right after Lemma~\ref{lem:sample-split-infinite-markov} that $\widehat{k}(s,a)\leq 665\tmix$. Taking the union bound over all integers $1\leq k\leq 665\tmix$ suffices to handle this statistical dependency. 

	\item In general, $\Daux$ and $\Dmain$ are statistically dependent as they are two parts of the same trajectory. 
		To resolve this issue, consider an additional collection of $S$ {\em independent} Markovian trajectories each of length $T/2$ (denoted by $\Daux(1), \Daux(2), \cdots, \Daux(S)$), where the $\Daux(s)$ starts from  state $s$ (note that these trajectories are introduced merely to assist in the proof). 
		Taking the union bound over all $s\in \cS$, we can establish the desired result, for every $s\in \cS$,  if the second dataset is $ \Daux(s)$. 
		Additionally, due to the Markovian property, we know that the true $\Daux$ must be statistically equivalent to one of these trajectories $\Daux(1), \cdots, \Daux(S)$; 
		this in turn establishes the claimed results for the true dataset.  

\end{itemize}
%
Putting everything together ensures the desired sample complexity as stated in Theorem~\ref{thm:infinite-markov}.

%as mentioned in Remark~\ref{remark:union}, to decouple the dependence between $\big\{\Ntrim_{\widehat{k}}(s, a)\big\}$ and $\Dmain$, it suffices to take a union bound over all the possible choices of $(s_{T/2}, \widehat{k})$, which introduce an additional factor of ${665S\tmix}$ in the logarithm term.
 
%
\end{proof}
 
		




==> models.tex <==
\section{Models and assumptions}
\label{sec:models}

In this section, we present the problem formulation along with the key assumptions.  





\subsection{Offline RL for discounted infinite-horizon MDPs}
\label{sec:models-infinite}

Next, we turn to the models and assumptions for discounted infinite-horizon MDPs. 

\paragraph{Basics of discounted infinite-horizon MDPs.}  Let us consider a discounted infinite-horizon  MDP \citep{bertsekas2017dynamic} represented by a tuple $\mathcal{M} = \{\cS, \cA, P, \gamma, r\}$. The key components of $\mathcal{M}$ are: (i) $\cS = \{1,2,\cdots, S\}$: a finite state space of size $S$; (ii) $\cA = \{1,2,\cdots, A\}$:  an action space of size $A$; (iii) $P: \cS\times \cA \rightarrow \Delta(\cS)$: the transition probability kernel of the MDP (i.e., $P (\cdot \mymid s,a)$ denotes the transition probability from state $s$ when action $a$ is executed); (iv) $\gamma \in [0,1)$: the discount factor, so that $\frac{1}{1-\gamma}$ represents the effective horizon; (v) $r: \cS\times \cA \rightarrow [0,1]$: the deterministic reward function (namely, $r(s,a)$ indicates the immediate reward received when the current state-action pair is $(s,a)$). Without loss of generality, the immediate rewards are normalized so that they are contained within the interval $[0,1]$.

\paragraph{Policy, value function and Q-function.}
A stationary policy $\pi: \cS \rightarrow \Delta(\cA)$ is a possibly randomized action selection rule; that is, $\pi(a \mymid s)$ represents the probability of choosing $a$ in state $s$. When $\pi$ is a deterministic policy, we abuse the notation by letting $\pi(s)$ represent the action chosen by the policy $\pi$ in state $s$. 
A sample trajectory induced by the MDP under policy $\pi$ can be written as $\{(s_t,a_t)\}_{t\geq 0}$, with $s_t$ (resp.~$a_t$) denoting the state (resp.~action) of the trajectory at time $t$. 
To proceed, we shall also introduce the value function $V^\pi$ and Q-value function $Q^\pi$ associated with policy $\pi$. Specifically, the value function $V^\pi: \cS \rightarrow \mathbb{R}$ of policy $\pi$ is defined as the expected discounted cumulative reward as follows:
%
\begin{align}
	\forall s\in\cS: \qquad 
	V^\pi(s) \coloneqq \mathbb{E} \left[\sum_{t=0}^\infty \gamma^t r(s_t, a_t) \mid s_0 = s; \pi\right],
	\label{eq:defn-Vpi-inf}
\end{align}
%
where the expectation is taken over the sample trajectory $\{(s_t, a_t)\}_{t\geq 0}$ generated in a way that $a_t \sim \pi(\cdot \mymid s_t)$ and $s_{t+1} \sim P(\cdot \mymid s_t, a_t)$ for all $t\geq 0$. Given that all immediate rewards lie within $[0,1]$, it is easily verified that $0\leq V^\pi(s) \leq \frac{1}{1-\gamma}$ for any policy $\pi$. The Q-function (or action-state function) of policy $\pi$ can be defined analogously as follows:
\begin{align}
	\forall (s,a)\in\cS \times \cA: \qquad 
	Q^\pi(s,a) \coloneqq \mathbb{E} \left[\sum_{t=0}^\infty \gamma^t r(s_t, a_t) \mid s_0 = s, a_0 = a; \pi\right],
\end{align}
%
which differs from \eqref{eq:defn-Vpi-inf} in that it is also conditioned on $a_0=a$. 




Let $\rho \in \Delta(\cS)$ be some (possibly unknown) initial state distribution. 
%Armed with above descriptions, we introduce several additional notations w.r.t~policy $\pi$.
If the initial state is randomly drawn from $\rho$, then we can define the following weighted value function of policy $\pi$:
%
\begin{align}
	V^\pi(\rho) \coloneqq \mathop{\mathbb{E}}\limits_{s\sim \rho}\big[V^\pi(s)\big].
\end{align}
%
In addition, we introduce the {\em discounted occupancy distributions} associated with policy $\pi$ as follows:
%
\begin{align}
	\forall s\in \cS: \qquad d^\pi(s; \rho) &\coloneqq (1-\gamma) \sum_{t=0}^\infty \gamma^t \mathbb{P}(s_t = s \mid s_0 \sim \rho;\pi),\\
	\forall (s,a)\in \cS \times \cA: \qquad d^\pi(s,a; \rho) &\coloneqq (1-\gamma) \sum_{t=0}^\infty \gamma^t \mathbb{P}(s_t = s, a_t =a \mid s_0 \sim \rho;\pi),
\end{align}
%
where we consider the randomness over a sample trajectory that starts from an initial state $s_0 \sim \rho$ and that follows policy $\pi$ (i.e., $a_t \sim \pi(\cdot \mymid s_t)$ and $s_{t+1} \sim P(\cdot \mymid s_t, a_t)$ for all $t\geq 0$).

As is well-known, there exists at least one deterministic policy --- denoted by $\pi^\star$ --- that simultaneously maximizes $V^\pi(s)$ and $Q^\pi(s,a)$ for all state-action pairs $(s,a)\in \cS\times \cA$ \citep{bertsekas2017dynamic}. We use the following shorthand notation to represent respectively the resulting optimal value and optimal Q-function:
%
\begin{align}
	\forall (s,a) \in \cS\times \cA: \qquad V^\star(s) \coloneqq V^{\pi^\star}(s) \quad \text{ and } \quad Q^\star(s,a) \coloneqq Q^{\pi^\star}(s,a).
\end{align}
%
Correspondingly, we adopt the notation of the discounted occupancy distributions associated with $\pi^\star$ as follows:
%
\begin{align}
	\forall (s,a) \in \cS\times \cA: \qquad d^\star(s) \coloneqq d^{\pi^\star}(s; \rho) \quad \text{ and } \quad 
	d^\star (s,a) \coloneqq d^{\pi^\star}(s,a; \rho) = d^{\star}(s) \ind\big( a = \pi^\star(s) \big),
\end{align}
%
where the last equality is valid since $\pi^\star$ is assumed to be deterministic.



\paragraph{Offline/batch single trajectory of data.}
%
Suppose that we have available a history dataset $\mathcal{D}$, which comprises a single trajectory of samples with length $T$ generated by a behavior policy $\pib$. More precisely, the sample sequence of the single trajectory takes the form
%
\begin{align}
	\{s_0, a_0, s_0, a_0,\cdots, s_T, a_T\},
\end{align}
%
which is generated by the MDP $\mathcal{M}$ in the following manner 
%
\begin{align}
	s_0 \sim \mu, \quad a_t \sim \pib(\cdot \mymid s_t),\quad s_{t+1} \sim P(\cdot \mymid s_t, a_t), \quad  0\leq t \leq T.
\end{align}
%
Note that the dataset $\mathcal{D}$ here consists of a single trajectory, thus resulting in substantially more complicated statistical dependency in comparison to a set of data drawn i.i.d.~from a simulator (as studied in \citet{rashidinejad2021bridging}). For notational convenience, we adopt the shorthand notation for the discounted occupancy distributions associated with $\pib$ as follows
%
\begin{align}
	\forall (s,a) \in \cS\times \cA: \qquad \myrho(s) \coloneqq d^{\pib}(s; \mu) \quad \text{ and } \quad
	\myrho (s,a) \coloneqq d^{\pib}(s,a; \mu).
\end{align}

%To characterize the distribution shift between the desired occupancy distributions and the occupancy distributions of the behavior policy, 

Akin to Assumption~\ref{assumption:concentrate-finite}, we introduce a certain concentrability assumption below to capture the distribution shift between the desired distribution and the one induced by the behavior policy. 
%
% the key concentrability for the infinite-horizon case which is weaker than the assumption in \citep{rashidinejad2021bridging}:
%
\begin{assumption}[Single-policy clipped concentrability for discounted infinite-horizon MDPs] 
\label{assumption:concentrate-infinite}
%
The batch dataset $\mathcal{D}$ satisfies
%
\begin{align}
	\max_{(s, a) \in \cS \times \cA}\frac{\min\big\{d^{\star}(s, a), \frac{1}{S}\big\}}{\myrho(s, a)} \le \Cstar
	\label{eq:concentrate-infinite}
\end{align}
%
for some quantity $\Cstar > 0$, with the convention that 0/0=0. We shall refer to the smallest $\Cstar$ satisfying \eqref{eq:concentrate-infinite} as the single-policy clipped concentrability coefficient. 
\end{assumption}
%
\begin{remark}
	As can be easily seen, the single-policy clipped concentrability coefficient $\Cstar$ can be viewed as a weaker condition compared to the single-policy concentrability coefficient $C^{\star}$ assumed in prior literature (e.g., \citet[Theorem 6]{rashidinejad2021bridging}), in the sense that   
	%
	\begin{equation}
		\Cstar \leq C^{\star}. \label{eq:Cstar-compare-inf}
	\end{equation}
	%
As we will see momentarily, this property \eqref{eq:Cstar-compare-inf} leads to improved performance guarantees. 
\end{remark}

\paragraph{Goal.} Armed with the batch dataset $\mathcal{D}$, the objective of offline RL in this case is to find a policy $\widehat{\pi}$ that attains near-optimal value functions in a sample-efficient manner, again with respect to a given test state distribution $\rho\in \Delta(\cS)$. 
To be precise, for any target accuracy level $\varepsilon \in (0,H]$, we seek to identify a near-optimal policy $\widehat{\pi}$ satisfying
%
\begin{align}
	V^\star(\rho) - V^{\widehat{\pi}}(\rho) \leq \varepsilon, 
\end{align}
%
using a batch dataset $\mathcal{D}$ of size as small as possible.






